Growing Tiny Networks: Spotting Expressivity Bottlenecks and Fixing Them Optimally

Machine learning tasks are generally formulated as optimization problems, where one searches for an optimal function within a certain functional space. In practice, parameterized functional spaces are considered, in order to be able to perform gradient descent. Typically, a neural network architecture is chosen and fixed, and its parameters (connection weights) are optimized, yielding an architecture-dependent result. This way of proceeding however forces the evolution of the function during training to lie within the realm of what is expressible with the chosen architecture, and prevents any optimization across architectures. Costly architectural hyper-parameter optimization is often performed to compensate for this. Instead, we propose to adapt the architecture on the fly during training. We show that the information about desirable architectural changes, due to expressivity bottlenecks when attempting to follow the functional gradient, can be extracted from backpropagation. To do this, we propose a mathematical definition of expressivity bottlenecks, which enables us to detect, quantify and solve them while training, by adding suitable neurons. Thus, while the standard approach requires large networks, in terms of number of neurons per layer, for expressivity and optimization reasons, we provide tools and properties to develop an architecture starting with a very small number of neurons. As a proof of concept, we show results~on the CIFAR dataset, matching large neural network accuracy, with competitive training time, while removing the need for standard architectural hyper-parameter search.

==> CIFAR10.tex <==
\begin{comment}
    
\subsection{CIFAR-10}
In this section we work with convolutional network  forward networks with an architecture of two blocks consisting of 2 convolutions and 1 MaxPooling each, followed by two fully-connected layers, using the $\mathrm{selu}$ activation function. The training criterion is the cross-entropy loss. 
We increase the size of the network on the fly (during training), with a batch size of $500$ for training using \ref{sec:batchsize_for_learning} on 1 GPU.
\subsubsection{About number of neurons and overfitting}
In Figure~\ref{fig:alpha9_2}, 100\% accuracy is achieved on training dataset, thus fully overfitting the data, which proves that  TINY can effectively bypass any expressivity bottleneck. Interestingly, this is done with fewer parameters than the theorem in \cite{zhang2017understanding}, which mentions $2n+d$ parameters to overfit a classification problem with $n$ samples of dimension $d$. This TINY architecture has about twice fewer parameters, 
due to generalization across samples, the labels in the CIFAR-10 classification task being not random.
It should also be noted that the TINY architecture  tends to overfit  less than the same final model retrained with all neurons from the beginning (FS), or at least, never more, which suggests that optimization and generalization abilities are not necessarily functions of neural network width anymore if one leaves the standard fixed-architecture training paradigm.
\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.28]{alpha_9_courbe_2.png}
    \caption{Experiment on CIFAR-10 dataset : Evolution of the train/test accuracy wrt gradient steps for TINY and FS}
    \label{fig:alpha9_2}
\end{figure}
\end{comment}


==> MNIST.tex <==
\subsection{MNIST}
In this section we work with feed forward networks with two hidden layers. We note by [$a, \;b$] such network with $a$ neurons on the first hidden layer and $b$ neurons on the second one. The experiments of this section are performed on 1 CPU. We use the optimizer $SGD(lr = 1e-3)$ and a starting batch size of 32  \ref{sec:batchsize_for_learning}. The training criterion is the cross-entropy loss and the activation function for the layers one and two is the Selu function.

The code for this section is at \textit{https://gitlab.inria.fr/mverbock/tinypub}.

\subsubsection{Random VS Optimization}\label{annexesec:random}
When performing the quadratic optimization (\ref{eq:probform}), we obtain the optimal direction for $({ \valpha}^*_k, { \vomega}^*_k)_{k = 1}^R$. It is also possible to generate randomly the new neurons and compute the amplitude factors on those. This second option have the benefit of being less time consuming, but it would project the desired direction on those random vectors and wouldn't affect the accuracy score compared to optimal solution defined in \ref{prop1}. 

In figure \ref{annexefig:TINY_vs_Random} we compare TINY and the Random method. We start with a network of size $[1, 1]$, we repeat five times the following process:
\begin{itemize}
    \item for each depth $d$:
    \begin{enumerate}
        \item Add neurons at layer $d$ with an amplitude factor.
        \item Perform the  best update at $d+1$ with an amplitude factor.
    \end{enumerate}
\end{itemize}
For the random method we generate the quantities of step 1. and 2. with a standard normal.
Then we evaluate the performance of the network on the test set. 
\begin{figure}[h]
    \centering
    \includegraphics[scale= 0.62]{TINY_vs_Random_MNIST.png}
    \caption{Box-plot of the accuracy on test set after adding neurons and performed best update at each layer. Experiment performed 10 times on the MNIST dataset.}
    \label{annexefig:TINY_vs_Random}
\end{figure}

%Adding random neurons speeds up the early learning when then size of the architecture is large. But it seems that the direction of random neurons are redundant with the structure of initial model because red models outperform green ones during training.
%\newpage
\subsubsection{Comparison with big model}\label{MNIST_bigalea}
On figure \ref{fig:TINY_Big}, we compare the time of training and the expressivity of a huge neural network of size $[1000, 1000]$ against a shallow neural which architecture is increased with the method TINY. 

We start with a network of size $[1, 1]$ and we increase its architecture by adding neurons with the TINY method with an amplitude factor at each layer. No best update is performed in this section. Each increase of architecture is followed by a training period of 0.1 epochs. Once the network has reached its final structure of $[26, 31]$, it is trained for few more steps, we note $s$ to total number of step on which the model is trained. We compared its performance with a huge network of size $[1000, 1000]$ which is trained for $s$ steps with all its neurons from scratch with a small batch size (the starting batch size for TINY, ie 32), BSbs,  or with a big batch size (the final batch size of TINY, ie 170), BBbs. Compared to the big model our TINY network converge as fast as the big ones because its architecture is smaller, converge slower in epochs because it is less expressive. 
\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.64]{TINY_vs_Big.png}
    \caption{\textit{(left)} Accuracy as a function of the time in seconds, \textit{(right)} accuracy as a function of gradient step. We plot mean and standard deviation for the same experiment repeated 5 times.\\}
    \label{fig:TINY_Big}
\end{figure}

%\begin{comment}
\subsubsection{Comparison with the same structure retrained from scratch}
In figure \ref{fig:MNIST_our_same_alea} we compare our method with a neural network retrained from scratch with the same architecture. 
\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.23]{comparaison_our_bigalea_7_10_12.png}
    \caption{
    %All graphics represent the values for accuracy on test of the same experiment but from a different perspective. \textbf{\textit{Left}} : after partitioning computational time on intervals of size $0.1$ seconds, we compute a linear interpolation for the accuracy value. \textbf{\textit{Middle}} : the accuracy value against number of epochs, where the time needed to compute the optimal neurons is not noticeable. \textbf{\textit{Right}} : accuracy against computational time, where durations due to Cholesky decompositions and their happening instants are averaged over experiments, for better visualisation purposes.\\.
    Accuracy on test set as a function of gradient step. Each plot correspond to one run.}
    \label{fig:MNIST_our_same_alea}
\end{figure}
%\end{comment}


==> lemma_norm_optimisation.tex <==
\begin{lemma}
    \label{lemma:fixed_norm_optimisation}
    Let $E$ an euclidean space, $F$ a subspace of $E$ and $\mY \in E$.

    \begin{equation}
        \min_{\mX \in F} \norm{\mY - \mX}^2 = \norm{\mY}^2 - \scalarp{\mY, \argmin_{\mX \in F} \norm{\mY - \mX}}
    \end{equation}
\end{lemma}

\begin{proof}
    Let $\mX \in F$. We note
    $\mD^* \in \argmax_{\mD \in F|\norm{\mD}=1} \scalarp{\mY, d}$ and $n^* := \scalarp{\mY, \mD^*}$. We first show that:
    \begin{equation}
        n^*\mD^* = \argmin_{\mX \in F} \norm{\mY - \mX}
    \end{equation}
    
    To do this, we show $\norm{\mY - n^* \mD^*} \leq \norm{\mY - \mX}$ or equivalently $\norm{\mY} - n^{*2} = \norm{\mY - n^* \mD^*}^2 \leq \norm{\mY - \mX}^2$.

    \begin{itemize}
        \item If $\mX \neq 0$:
        We have:
        \begin{align}
            \norm{\mY - \mX}^2
            &= \norm{\mY}^2 - 2 \scalarp{\mY, \mX} + \norm{\mX}^2 \\
            &= \norm{\mY}^2 - 2 \norm{\mX} \scalarp{\mY, \frac{\mX}{\norm{\mX}}} + \norm{\mX}^2 \\
            &\geq \norm{\mY}^2 - 2 \norm{\mX} \max_{\mD \in F|\norm{\mD}=1} \scalarp{\mY, \mD} + \norm{\mX}^2
        \end{align}
        
        \item If $\mX = 0$:
        \begin{align}
            \norm{\mY - \mX}^2
            &= \norm{\mY}^2 - 2 \norm{\mX} \scalarp{\mY, \mX} + \norm{\mX}^2 \\
            &\geq \norm{\mY}^2 - 2 \norm{\mX} \max_{\mD \in F|\norm{\mD}=1} \scalarp{\mY, \mD} + \norm{\mX}^2
        \end{align}
    \end{itemize}

    Then we can conclude the first goal, with the same reasoning for both cases:
    \begin{align}
        \norm{\mY - \mX}^2
        &\geq \norm{\mY}^2 - 2 \norm{\mX} \scalarp{\mY, \mD^*} + \norm{\mX}^2 \\
            &\geq \min_{\mZ \in F} (\norm{\mY}^2 - 2 \norm{Z} \scalarp{\mY, \mD^*} + \norm{\mZ}^2) \\
            &= \min_{||\mZ||\geq 0} (\norm{\mY}^2 - 2 \norm{Z} n^* + \norm{\mZ}^2) \\
            &= \norm{\mY}^2 - n^{*2}
    \end{align}

    Hence:
    \begin{align}
        \min_{\mX \in F} \norm{\mY - \mX}^2
        &= \norm{\mY}^2 - n^{*2}\\
        &= \norm{\mY}^2 - n^*\scalarp{\mY, \mD^*}\\
        &= \norm{\mY}^2 - \scalarp{\mY, n^* \mD^*}
    \end{align}

\end{proof}


==> lemma_scalap_value_old.tex <==
\begin{lemma}
    \label{lemma:scalarp_value1}
    We note $\mDE (\mA, \mOmega)$ the result of $B$ after applying the layers parameterized by $\mA$ and $\mOmega$ and $\mDE ^* = \mDE (\mA^*, \mOmega^*)$.

    \begin{equation}
        \scalarp{\mDV_{proj}, \mDE^*} \geq \norm{\Lambda_{k}}^2
    \end{equation}
    with an equality in the case of fully connected layers.
\end{lemma}
\begin{proof}
    First using~\cref{lemma:linear_quadratic_problem},~\cref{lemma:conv_quadratic_problem} and~\cref{lemma:optimal_neurons}, we have:
    \begin{align}
        \min_{\mA, \mOmega} \norm{\mDE (\mA, \mOmega) - \mDV_{proj}}^2 
        &\leq \min_{\mA, \mOmega} \norm{\Shalf \mA \mOmega - \Smhalf\mN}^2  - \norm{\Smhalf\mN}^2 + \norm{\mDV_{proj}}^2\\
        &= \norm{\Lambda_{k+1:}}^2 - \norm{\Lambda}^2 + \norm{\mDV_{proj}}^2 \\
        &= -\norm{\Lambda_k}^2 + \norm{\mDV_{proj}}^2
    \end{align}
    with an equality in the case of fully connected layers.

    On the other hand, $\set{\mDE (\mA, \mOmega) | \mA, \mOmega}$ is a vector subspace. Using~\cref{lemma:fixed_norm_optimisation}, we have:
    \begin{equation}
        \min_{\mA, \mOmega} \norm{\mDE (\mA, \mOmega) - \mDV_{proj}}^2 = \norm{\mDV_{proj}}^2 - \scalarp{\mDV_{proj}, \mDE_{opt}}
    \end{equation}
    where $$V_{opt} := \argmin_{V = V(\mA, \mOmega)} \norm{V - \mDV_{proj}}$$

    Hence we have:
    \begin{equation}
        \norm{\Lambda_k}^2 \leq \scalarp{\mDV_{proj}, \mDE_{opt}}
    \end{equation}
    (with an equality in the case of fully connected layers.)
\end{proof}


==> old_part_5_greedy_growth.tex <==

\section{About greedy growth sufficiency}\label{greedy}

One might wonder whether a greedy approach on layer growth might get stuck in a non-optimal state. By \emph{greedy} we mean that every neuron added has to decrease the loss. 
%We derive the following series of propositions in this regard, proving the existence of greedy growth strategies with good properties. 
Since in this work we add neurons layer per layer independently, we study here the case of a single hidden layer network, to spot potential layer growth issues. For the sake of simplicity, we consider the task of least square regression towards an explicit continuous target $f^*$, defined on a compact set. That is, we aim at minimizing the loss:\vspace{-2mm}
$$\inf_f \sum_{x \in \mathcal{D}} \|f(x)-f^*(x)\|^2$$
where $f(x)$ is the output of the neural network and $\mathcal{D}$ is the training set. Proofs are deferred to Appendix \ref{sec:greedyproof}, as well as supplementary propositions.

%\subsection{Possibility of greedy growth}

\begin{prop}[Greedy completion of an existing network] If $f$ is not $f^*$ yet, 
%for any arbitrarily small desired  precision $\epsilon$, 
then there exists a set of neurons to add to the hidden layer such that the new function $f'$ will have a lower loss than $f$.
\end{prop}
One can even choose the added neurons such that the loss is arbitrarily well minimized. Furthermore:

\begin{prop}[Greedy completion by one single neuron]
 If $f$ is not $f^*$ yet, there exists a neuron to add to the hidden layer such that the new function $f'$ will have a lower loss than $f$.
\end{prop}
As a consequence, there exists no situation where one would need to add many neurons simultaneously to decrease the loss: it is always feasible with a single neuron.
Note that finding the optimal neuron to add is actually NP-hard~\citep{bach2017breaking}, so we will not necessarily search for the optimal one.
%One can express 
A constructive lower bound on how much the loss can be improved will be given later in this section. %(for the best such neuron), but it is not a very good bound without further assumptions on $f$. Furthermore,

\begin{prop}[Greedy completion by one infinitesimal neuron]\label{prop:infinit}
The neuron in the previous proposition can be chosen to have arbitrarily small input weights.
\end{prop}
This detail is important in that our approach is based on the tangent space of the function $f$ and thus manipulates infinitesimal quantities. 
%Though we perform line search in a second step and consequently add non-infinitesimal neurons, our first 
Our optimization problem indeed relies on the linearization of the activation function by requiring the added neuron to have infinitely small input weights,
%without which it would be much harder to solve.
to make the problem easier to solve.
This proposition confirms that such neuron exists~indeed.

\paragraph{Correlations and higher orders.}
%Note that this proposition does not state that our approach will find that neuron. Indeed, 
Note that, as a matter of fact, our approach exploits
%we exploit 
linear correlations between inputs of a layer and desired output variations. It might happen that the loss is not minimized yet but there is no such correlation to exploit anymore. In that case the optimization problem (\ref{eq:probform}) will not find neurons to add. Yet following Prop.~\ref{prop:infinit} there does exist a neuron with arbitrarily small input weights that can reduce the loss. This paradox can be explained by pushing further the Taylor expansion of that neuron output in terms of weight amplitude (single factor $\epsilon$ on all of its input weights), for instance
%contains no linear term but a quadratic or higher-order one: 
$\sigma(\epsilon {\boldsymbol\alpha}\cdot \vx) \simeq \sigma(0) + \sigma'(0) \epsilon {\boldsymbol\alpha}\cdot \vx + \frac{1}{2} \sigma''(0) \epsilon^2 ({\boldsymbol\alpha}\cdot \vx)^2 + O(\epsilon^3)$.
Though the linear term ${\boldsymbol\alpha}\cdot \vx$ might be uncorrelated over the dataset with desired output variation $v(\vx)$, i.e.~$\E_{\vx\sim\mathcal{D}}[ \vx \, v(\vx)] = 0$, the quadratic term $({\boldsymbol\alpha}\cdot \vx)^2$, or higher-order ones otherwise, might be correlated with $v(\vx)$. Finding neurons with such higher-order correlations can be done by increasing accordingly the power of $({\boldsymbol\alpha}\cdot \vx)$ in the optimization problem (\ref{eq:eq_rajout}). Note that one could consider other function bases than the polynomials from Taylor expansion, such as Hermite or Legendre polynomials, for their orthogonality properties.
In all cases, one does not need to solve such problems exactly but just to find an approximate solution, i.e.~a neuron improving the loss.
%The complexity of the problem is increased as well,

%We would have to move to higher-order changes, that is for instance to exploit correlations with squared inputs, etc.

%\subsection{Exploiting linear correlations vs. exploring high-orders with random neurons}

\paragraph{Adding random neurons.} Another possibility to suggest additional neurons, when expressivity bottlenecks are detected but no correlation (up to order $p$) can be exploited anymore, is to add random neurons. The first $p$ order Taylor expansions will show 0 correlation with desired output variation, hence no loss improvement nor worsening, but the correlation of the $p+1$-th order will be non-0, with probability 1, in the spirit of random projections. 
%This provides a loss improvement direction. 
%The loss can then be improved, all the more with a line search to optimize the neuron amplitude.
%%Yet, such improvement from random neurons is hindered by the directions in the functional space other than the desired one to which the neuron contributes
%However, such random neurons also contribute to other directions in the functional space than the desired one. This hinders the loss improvement expectable from them, as the line search will need to find a compromise with the loss changes brought by these other directions. This is confirmed experimentally in Appendix \ref{annexesec:random}.
%To alleviate this, i
Furthermore, in the spirit of common neural network training practice, one could consider brute force combinatorics by adding many random neurons and hoping 
%that one 
some
will be close enough to the desired direction~\citep{DBLP:journals/corr/abs-1803-03635}.
%\todo{ cite ticket Lot}. 
The difference with usual training is that we would perform such computationally-costly searches only when and where relevant, exploiting all simple information first (linear correlations~in~each~layer). 

%So far, on our experiments on MNIST, we actually do not see any problematic situation requiring such extra care; experiments on harder tasks and bigger networks are needed to confirm this tendency.

\paragraph{Reaching 0 training loss.} We now constructively show that 0 training error can be reached by greedy growth. %, i.e., growth where each neuron addition decreases the training loss. 
For this, we quantify the expected loss gain at each neuron addition, or the number of neuron additions required to reach 0 training loss, depending on the allowed operations. In both cases below, 
%we consider the case of a mean square regression, using a single-hidden-layer fully-connected neural network
a supplementary hypothesis is that activation functions are ReLU.
Constructive proofs can be found in Appendices \ref{app:expconv} and \ref{app:reaching}, respectively.

\begin{prop}[Exponential convergence to 0 training error by neuron additions and line search]  
It is possible to decrease the loss exponentially fast with the number $t$ of added neurons, i.e.~as $\gamma^t \gL(f)$, towards 0 training loss, and this in a greedy way, that is, such that each added neuron decreases the loss. The factor $\gamma$ is $\gamma = 1 - \frac{1}{n^3 d'} \left(\frac{d_m}{d_M}\right)^2$, where $d_m$ and $d_M$ are quantities solely dependent on the dataset geometry, and $d'$ is the output dimension of the network.
\end{prop}

\begin{prop}[Reaching 0 training error in $n$ neuron additions when jointly updating existing output weights] 
If one allows updating already existing output weights at the same time as one adds new neurons, then it is possible to reach 0 training error in only $n$ steps (where $n$ is the size of the dataset) while decreasing the loss at each addition.
\end{prop}

This scenario is closer to the one we consider with TINY, as we compute the optimal update of existing weights inside the layer, as a byproduct of new neuron estimation, and apply them. The way to build new neurons is different though. Our approach shares similarity with gradient boosting \cite{friedman2001greedy} somehow, as we grow the architecture based on the gradient of the loss.

==> part_5_5_resultat.tex <==
\section{Results}
\label{sec:results}
%In this section w
We evaluate our method, called \textbf{TINY}, on the CIFAR-10 dataset 
\citep{krizhevsky2009learning}.
%\citep{CIFAR10}. 
We start with an architecture of two blocks consisting of 2 convolutions and 1 MaxPooling each, followed by two fully-connected layers, using the
%Each convolutional block is made of two convolutional layers and ends by one MaxPooling. 
%The activation function for the convolutional and linear layers is
the $\mathrm{selu}$
activation function.
%function and w
The training criterion is the cross-entropy loss. 
We
%Our method 
increase the size of the network on the fly (during training), with a batch size of $500$ for training, see \ref{sec:batchsize_for_learning}. More experiments can be found in Appendix \ref{additionalresult}.

In Figure \ref{fig:Our_GM_RP_T_eq_0_500}, the TINY method is compared to GradMax (\textbf{GM})~\citep{evci2022gradmax}
We imitate 
%replicate the results of
this method by skipping the projection step of the desired update on the current architecture.
%and (2) by replacing the desired update by a random vector for \textbf{RP}. For a detailed explanation of these choices, please refer to~\ref{sec:theorical_comparaison}.
% We mimic those methods by not projecting the desired update on the current architecture for \textbf{GM} and by replacing the desired update by a random vector for \textbf{RP} (for more details see \ref{sec:theorical_comparaison}).
The \textit{Left} and \textit{Right} plot respectively correspond to the plots of the accuracy $acc_0$ on validation set after adding all the neurons,  and the accuracy $acc_{\infty}$ at the end of training. On the $x$-\textit{axis}, we measure the complexity of each model  as the number of basic operations performed during test.

At a fixed complexity, before and after the final training, our method out-performs GradMax because of the redundancy of that procedure. While GradMax neurons align with the gradient when expressivity  bottlenecks can be mostly  solved by the current architecture, we add new directions and decrease the expressivity bottleneck as defined in (\ref{eq:mini_NG}) by projecting the desired update. In the GradMax paper, to avoid redundancy, neurons can be added only once the gradient of the current structure vanishes to $0$. Our method allows to skip this waiting by projecting the desired update on the current structure using (\ref{eq:dwl}).

 In Figure~\ref{fig:alpha9} we compare our results with a baseline (\textbf{FS}) where the final TINY architecture is retrained from start with a new set of weights, initialized with Xavier Normal distribution and trained until convergence. The Figure shows the evolution of train/test accuracy for the TINY and from scratch (\textbf{FS}) methods. No new neurons are added after 4000 steps in TINY. It is possible to achieve 100\% accuracy on training dataset, thus overfitting the data, meaning that TINY could effectively bypass any expressivity bottleneck,
and this with fewer parameters than \citep{zhang2017understanding}'s theorem. 
%Figure \ref{fig:alpha9} proove that our method yields better or similar performance than the \textit{optimal architecture}.
While usual methods have to train until convergence different architectures to find the optimal one, our method achieves this result in a single run. 

%In the second experiment we compare our method  with a baseline (\textbf{FS}) where the final TINY architecture is retrained from start with a new set of weights initialized with Xavier Normal distribution. \\
\section{Limitations}
At a given layer, our method reduces expressivity bottlenecks, unless the required information has been lost in previous layers. This situation might arise e.g.~with very thin, deep neural networks, especially with ReLU activations. In such a case, the lack of information flow might prevent any update. This limitation however disappears if using skip connections or if new layers can be added to the architecture. In Appendix \ref{sec:cifar100} we are thus able to train a ResNet-18 model on CIFAR-100.

%as one progresses through the different layers, an increasingly larger portion of the input space is mapped to 0 because each layer divides the input space with a hyperplane, resulting in 0 on one side of this hyperplane and a linear function on the other side \citep{DBLP:journals/corr/abs-1810-07481}. This phenomenon may push matrices $S$ and $N$ to 0, as well as the estimated gain of loss $\lambda_k^2$. To mitigate this issue, it would be beneficial to establish connections between layers, such as skip connections, which is a task we intend to address in future work.

%At a given layer, our method can reduce the expressivity bottlenecks if the information has not being lost at previous layer. This occurs when starting with thin deep neural network with $\textit{relu}$ as the activation function.
%with few neurons at each layer and considering layer close to the output, 
%The gain of loss associated to the new neurons computed by \ref{prop2}, ie $(\lambda_k)_K$,  will be poor as the information contained in $\vb_{l-2}$ is not usable. a deep feed-forward network with only one neuron by layer and $\textit{relu}$ as the activation function.
%In this setting, as we pass through the different layers, an ever-increasing share of the input space is mapped into $0$ because each layer cut the input space with a hyperplane and output $0$ on one side of this hyperplane and a linear function on the other side \citep{DBLP:journals/corr/abs-1810-07481}. It would push the matrix $\mS$ and $\mN$  to $0$ as well as the $\lambda_k$. This problem can be bypass if the layers were not only connected to their collaterals (skip connections) a task we leave for future work.
\section{Conclusion}%\vspace{-1mm}
We have properly defined lacks of expressivity, and their minimization has allowed us to optimize the architecture on the fly, to better follow the functional gradient, enabling architecture growth,
%We were thus able to train greedily tiny architectures without facing extra
and escaping
optimization issues usually associated to layer thinness.
Work in progress includes the extension to layer addition in order to  fully automatically develop architectures, a statistical test to assess the significance of estimated neurons to add, 
and a strategy for neuron addition based on a compromise between performance gain and added computational complexity.
%to compare the gain of performance of the new neurons and the expressivity of the current architecture.


\begin{figure}[h!]
    \begin{minipage}{0.5\columnwidth}
        \centering
    \includegraphics[scale = 0.41]{Our_GM_RP_T_eq_0.png}
    %\label{fig:Our_GM_RP_T_eq_0}
    \end{minipage}
    \begin{minipage}{0.45\columnwidth}
        \centering
    \includegraphics[scale = 0.41]{Our_GM_RP_T_eq_500.png}
    \end{minipage}
    \vspace{-2mm}
    \caption{Experiments on CIFAR Dataset: accuracies (\textit{Left}) $acc_0$, (\textit{Right}) $acc_{\infty}$ on test set against the complexity for \textbf{GM} and \textbf{Our} method. The starting architecture $N_{init}$ has the structure of 3 neurons per convolutional layers and 5 neurons per linear layer which is of complexity $2\times 10^5$.}
    \label{fig:Our_GM_RP_T_eq_0_500}%\vspace{-2mm}
    
\end{figure}

%The point cloud of figure \ref{fig:Our_GM_RP_T_eq_0} and \ref{fig:Our_GM_RP_T_eq_infty} is obtained with the pseudo-code :
%\vspace{-4mm}
\newcommand{\NN}{$N\!N$}
%\begin{figure}[h!]%\vspace{-8mm}
\begin{algorithm}[H]
% Initialize a small neural network $N_{init}$ \;
 \For{each method [Ours, GradMax]}{
    Start from a given small neural network \NN \;
%    Clone $N_{init}$ into $N_{method}$\;
    \For{j in $nb_{pass}$}{
    \For{each layer $l$}{
    Compute the first three neurons to add at layer $l$ \; 
    $\;\;\;\;\;$ // \emph{with our method the above also yields $\delta  \mW_l^*$ as a by-product}\;
    Select among them the ones with significant singular value (Appendix \ref{eigenvalues_significance})\;
    Compute the amplitude factor $\gamma$ for the new neurons (Appendix \ref{sec:amplitude_facteur}) \;
    Add the neurons if $\gamma > 0$\;
    Update the architecture with the best update $\delta  \mW_l^*$ at $l\!+\!1$ (only for our method)
    }
    }
    Get accuracy $acc_0$ of \NN\;
    Train \NN for 15 epochs \;
    Get final accuracy $acc_{\infty}$ of \NN\;
 }
\caption{Algorithm to plot Figure \ref{fig:Our_GM_RP_T_eq_0_500}.}%\vspace{-4mm}
\label{algo_plot}%\vspace{-2pt}
\end{algorithm}%\vspace{-3mm}
%\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[scale = 0.3]{alpha_9_courbe_1.png}%\vspace{-2mm}
    \caption{Evolution of the train/test accuracy wrt gradient steps for TINY and FS.}\vspace{-5mm}
    \label{fig:alpha9}
\end{figure}%\vspace{-4pt}

%\newpage


\begin{comment}

We start with an architecture with 3 (resp. 20) neurons on the convolutional (resp. linear) layers. We add 10 neurons on each convolutional layer and 10 neurons on the linear layer. 
In order to see better the difference of impact of each method we multiply the fan-in weights of the new neurons with an amplitude factor, \emph{i.e.} $\alpha \xleftarrow{} \epsilon \alpha$. The amplitude factor $\epsilon$ is chosen such that it decreases the most of the loss on the train dataset.
The figure~\ref{fig:GM_RP_Our} shows the relative increase of accuracy averaged for all added neurons. It appears that the NorthPreactivation (RP) method, which adds randomly initialized neurons, does not increase the accuracy on training or on test set. The GM and TINY methods add a clear improvement on both the training and test accuracy, and the TINY yields better results than GM. Also, contrary to the GM method, TINY  does not need to wait for gradient convergence when adding neuron to avoid redundancy. Actually, the GM method does not explicitly take into account redundancy in the network and furthermore does not provide an objective criterion for neuron 
selection or model size.
%addition. %to know if one must add a neuron or not.
% comparaison avec GradMax, on fait mieux en accuracy (cf figure 8 dans  et on plus on a pas besoin d'attendre la convergence du gradient et en plus il se fichent de la redondance du réseau. Pas de critère pour savoir s'il faut ajouter des neurones ou pas.

In the second experiment, we demonstrate the effectiveness of our selection criterion to grow the architecture.
We start with an architecture of one (resp. five) neurons for the convolutional (resp. linear) layer. 
We compare our results with a baseline (\textbf{FS}) where the final TINY architecture is retrained from start with a new set of weights, initialized with Xavier Normal distribution and trained until convergence. %This baseline method is called  and is trained until convergence. 
We evaluated several architecture growth by varying the weight $\alpha$ of the computation time penalty, using values in $\left[ 1e^{-8}, 1e^{-9}\right]$. The accuracy score is assessed using early stopping on the validation set. The figure~\ref{fig:Pareto} shows that we obtain the same or better accuracy for equivalent time complexity with our TINY method. This demonstrates that TINY grows very small network into an optimal architecture that captures observed variability in the training dataset.
The Figure~\ref{fig:alpha9} shows the evolution of train/test accuracy for the TINY and FS methods. No new neurons are added after 4000 steps in TINY, as the selection criterion is not met anymore. It is possible to achieve 100\% accuracy on training dataset, thus overfitting the data, meaning that TINY could effectively bypass any expressivity bottleneck,
and this with fewer parameters than \citep{zhang2017understanding}'s theorem. 

%compare our method selection (\textbf{TINY}) with the classic method (\textbf{FS}) on CIFAR-10 database \citep{CIFAR10} with figure \ref{graph:pareto} while we compare with GradMax method of paper \citep{evci2022gradmax} and with  NorthPreactivation of paper \citep{maile2022when} in figure \ref{fig:GM_PR_Our}.
%   For our method our method \textbf{TINY} we start with an architecture  of two VGG blocks followed by two linear layers. Each VGG block is made of two convolutional layers and ends by one MaxPooling. The starting architecture is one, five neurons by resp. convolutional, linear layer. The activation function for the linear and convolutional layers is the $selu$ function and we compute the loss using the cross-entropy loss. While our method increases the size of the network training, the \textbf{FS} method start with last/(or one of architecture) tried architecture and is trained until convergence.  The starting batchsize is $100$, see \ref{sec:batchsize_for_learning}. 
%    For our method our method \textbf{TINY} we start with an architecture  of two VGG blocks followed by two linear layers. Each VGG block is made of two convolutional layers and ends by one MaxPooling. The starting architecture is one, five neurons by resp. convolutional, linear layer. The activation function for the linear and convolutional layers is the $selu$ function and we compute the loss using the cross-entropy loss. While our method increases the size of the network training, the \textbf{FS} method start with last/(or one of architecture) tried architecture and is trained until convergence.  The starting batchsize is $100$, see \ref{sec:batchsize_for_learning}. 
    
%\begin{minipage}{0.5\columnwidth}
\begin{figure}
    \begin{minipage}{.28\textwidth} %[c][11cm][t]
        \vspace*{\fill}
        \centering
        \includegraphics[width=0.98\linewidth]{GM_RP_Our.png}    
        \subcaption{accuracy improvement}
        \label{fig:GM_RP_Our}
    \end{minipage}
    \begin{minipage}{.71\textwidth} %[c][t]
        \vspace*{\fill}
        \centering
        \includegraphics[width=0.98\linewidth]{Pareto.png}
        \subcaption{accuracy-time complexity tradeoff}
        \label{fig:Pareto}\par\vfill
        \includegraphics[width=0.98\linewidth]{alpha_9_courbe_1.png}
        \subcaption{Architecture evolution}
        \label{fig:alpha9}
    \end{minipage}
    
    %\centering
    %\includegraphics[width=0.25\linewidth]{GM_RP_Our.png}
    %\includegraphics[width=0.72\linewidth]{Pareto.png}
    %\includegraphics[width=0.72\linewidth]{alpha_9_courbe_1.png}
    \caption{(A) The marker corresponds to the mean/std accuracy improvement when adding neurons. (B) Accuracy on the test set depending on time complexity. (C) Evolution of the train/test accuracy wrt gradient steps for TINY and FS.\vspace{-4mm}}
\end{figure}
%\end{minipage}

%\begin{minipage}{0.49\columnwidth}
%    We mimic those methods by not projecting the desired update on the current architecture for \textbf{GM} and by replacing the desired update by a random vector for \textbf{RP} (for more details see \ref{sec:theorical_comparaison}).

%\end{minipage}

%\begin{minipage}{0.4\columnwidth}
%\begin{algorithm}[H]
% \For{j=1, ..., k }{
%  \For{l = 1, ..., depth - 1}{
%   loop($l$, SM = '\textbf{RTM}')\;
%   }
%  }
%  model.train(epochs = 10)\;
% \caption{Expand}
%\end{algorithm}

%\end{minipage}
%\fbox{
%\begin{figure}
%\begin{minipage}{0.6\columnwidth}
    %\centering
%    \begin{centering}
%    \includegraphics[scale = 0.5]{Pareto.png}
%    \caption{Acuuracy on test set as a function of the time complexity}  %In blue, projection of $\textcolor{teal}{\displaystyle \vDV}$ on $\TA$.
%    \end{centering}
%    \label{graph:pareto}
%\end{minipage}
%\end{figure}
    
\end{comment}

% faire un renvoi vers la figure de 10h49 et 14h10 dans les annexes pour montrer l'ajout 
%\newpage


